Data-Dependent Coresets for Compressing Neural Networks with Applications to Generalization Bounds

We present an efficient coresets-based neural network compression algorithm that sparsifies the parameters of a trained fully-connected neural network in a manner that provably approximates the network's output. Our approach is based on an importance sampling scheme that judiciously defines a sampling distribution over the neural network parameters, and as a result, retains parameters of high importance while discarding redundant ones. We leverage a novel, empirical notion of sensitivity and extend traditional coreset constructions to the application of compressing parameters. Our theoretical analysis establishes guarantees on the size and accuracy of the resulting compressed network and gives rise to generalization bounds that may provide new insights into the generalization properties of neural networks. We demonstrate the practical effectiveness of our algorithm on a variety of neural network configurations and real-world data sets.

==> related-work-before-iclr.tex <==
\section{Related Work}
\label{sec:related-work}
Our work builds upon the following prior work in coresets and compression approaches.

\CB{Emphasize that we don't need retraining}
\paragraph{Coresets} 
Coreset constructions were originally introduced in the context of computational geometry \citep{agarwal2005geometric} and subsequently generalized for applications to other problems via an importance sampling-based, \emph{sensitivity} framework~\citep{langberg2010universal,feldman2011unified,braverman2016new}. Coresets have been used successfully to accelerate various machine learning algorithms such as $k$-means clustering~\citep{feldman2011unified,braverman2016new}, graphical model training~\citep{molina2018core}, and logistic regression~\citep{huggins2016coresets} (see the surveys of~\citep{bachem2017practical,munteanu2018coresets} for a complete list). In contrast to prior work, we generate coresets for reducing the number of parameters -- rather than data points -- via a novel construction scheme based on an efficiently-computable notion of sensitivity.

\paragraph{Low-rank Approximations and Weight-sharing}
\citet{Denil2013} were among the first to empirically demonstrate the existence of significant parameter redundancy in deep neural networks. A predominant class of compression approaches consists of using low-rank matrix decompositions, such as Singular Value Decomposition (SVD)~\citep{Denton14}, to approximate the weight matrices with their low-rank counterparts. Similar works entail the use of low-rank tensor decomposition approaches applicable both during and after training~\citep{jaderberg2014speeding, kim2015compression, tai2015convolutional, ioannou2015training, alvarez2017compression, yu2017compressing}. Another class of approaches uses feature hashing and weight sharing~\citep{Weinberger09, shi2009hash, Chen15Hash, Chen15Fresh, ullrich2017soft}. Building upon the idea of weight-sharing, quantization~\citep{Gong2014, Wu2016, Zhou2017} or regular structure of weight matrices can be used for reducing the effective number of parameters~\citep{Zhao17, sindhwani2015structured, cheng2015exploration, choromanska2016binary, wen2016learning}. Despite their favorable empirical effectiveness in compressing neural networks, these works generally lack performance guarantees on the quality of their approximations and/or the size of the resulting compressed network.

\paragraph{Weight Pruning}
Similar to our proposed method, weight pruning~\citep{lecun1990optimal} hinges on the idea that only a few dominant weights within a layer are required to approximately preserve the output. Approaches of this flavor have been investigated by~\cite{lebedev2016fast,dong2017learning}, e.g., by embedding sparsity as a constraint~\citep{iandola2016squeezenet, aghasi2017net, lin2017runtime}. Another related approach is that of~\cite{Han15}, which considers a combination of weight pruning and weight sharing methods. %
%To the best of our knowledge, our work is the first to introduce a practical, sampling-based weight pruning algorithm with provable guarantees.
However, prior work in weight pruning lacks rigorous theoretical analysis of the effect that the discarded weights can have on the compressed network. 

\paragraph{Generalization}
The generalization properties of neural networks have been extensively investigated in various contexts~\citep{dziugaite2017computing, neyshabur2017pac, kawaguchi2017generalization, bartlett2017spectrally}. However, as was pointed out by~\cite{zhang2016understanding} and~\cite{neyshabur2017exploring}, current approaches to obtaining non-vacuous generalization bounds do not fully or accurately capture the empirical success of state-of-the-art neural network architectures.
Recently, \cite{arora2018stronger} and \cite{zhou2018compressibility} highlighted the close connection between compressibility and generalization of neural networks. \cite{arora2018stronger} presented a compression method based on the Johnson-Lindenstrauss (JL) Lemma~\citep{johnson1984extensions} and proved generalization bounds based on succinct reparameterizations of the original neural network. Building upon the work of~\cite{arora2018stronger}, we extend our theoretical compression results to establish novel generalization bounds for fully-connected neural networks.

In contrast to prior work, this paper addresses the problem of \emph{provably} compressing a fully-connected neural network while preserving the output for any point from the data distribution up to any user-specified approximation accuracy and failure probability.  Unlike the method of~\cite{arora2018stronger}, which exhibits guarantees of the compressed network's performance only on the set of training points, our method's guarantees hold for any point drawn from the distribution. 



==> related-work-old.tex <==
% A FEW OLD PARAGRAPHS FROM RELATED WORK 

\paragraph{Coresets}
Coreset constructions were introduced in the context of computational geometry \citep{agarwal2005geometric} and subsequently generalized for applications to other problems via an importance sampling-based, \emph{sensitivity} framework that was originally introduced by~\citep{langberg2010universal} and later improved by~\citep{feldman2011unified} and~\citep{braverman2016new}. Coresets have been applied to and enjoyed widespread success in accelerating a diverse set of machine learning algorithms including $k$-means clustering~\citep{feldman2011unified,braverman2016new}, mixture model training~\citep{feldman2011scalable,lucic2017training}, dependency network  training~\citep{molina2018core}, and logistic regression~\citep{huggins2016coresets} (see the surveys of~\citep{bachem2017practical,munteanu2018coresets} for a more complete list). In contrast to prior work, we generate coresets for reducing the number of parameters rather than training data points by a novel approach based on an empirical notion of sensitivity. In comparison to traditional coreset constructions, our coreset generation scheme leverages the training data set to efficiently compute accurate approximations of the relative importance of each parameter, leading to informed parameter sampling and provably small coreset sizes.

\paragraph{Neural Network Compression} Denil et al.~\cite{Denil2013} were among the first to empirically establish that there is significant redundancy in the parameters of deep neural networks. Thus, a significant amount of research over the last years has been devoted to network compression. A predominant class of approaches is that of using low-rank matrix decompositions to approximate the weight matrices. A method for achieving this based on the Singular Value Decomposition (SVD) was presented in \cite{Denton14} and inspired numerous works on low-rank tensor decomposition approaches applicable both during and after training~\cite{jaderberg2014speeding,kim2015compression,tai2015convolutional,ioannou2015training,alvarez2017compression,yu2017compressing}. Another class of approaches uses feature hashing and weight sharing~\cite{Weinberger09,shi2009hash,Chen15Hash,Chen15Fresh,ullrich2017soft}. Building upon the idea of weight-sharing, regular structure of weight matrices can be used for reducing the effective number of parameters~\cite{Zhao17,sindhwani2015structured,cheng2015exploration,choromanska2016binary,wen2016learning}. Despite their favorable empirical effectiveness in compressing neural networks, virtually of these works provide no performance guarantees on the quality of their approximations and/or the size of the resulting compressed network.

\paragraph{Weight pruning}
Similar to our proposed method, the premise of weight pruning is to reduce the number of effective parameters by sparsifying the weight matrices with the overarching goal of reducing storage requirements and accelerating inference. Originally introduced by LeCun et al.~\cite{lecun1990optimal}, weight-sharing hinges on the idea that among the multitude of weights constituting a weight matrix associated with a layer, only a few dominant weights will significantly affect the output of the neural network, whereas the remaining weights are deemed for the most part redundant. Therefore, only the small number of important weights can be kept and the remaining weights can be pruned.

Approaches of this flavor have been investigated in~\cite{lebedev2016fast,dong2017learning}, however, prior work has not considered rigorously analyzing the theoretical properties of these approaches. Similarly, ~\cite{lin2017runtime} and~\cite{aghasi2017net,iandola2016squeezenet} proposed methods where sparsity is explicitly embedded as an optimization objective during training. Another related approach is that of~\cite{Han15}, which considers a combination of weight pruning and weight sharing methods. In contrast to these approaches, to the best of our knowledge, our work is the first to introduce a practical, sampling-based weight pruning algorithm with provable guarantees that imposes minimal assumptions on the neural network weights and input data distribution.

\paragraph{Generalization} Recently, Arora et al.~\cite{arora2018stronger} and Zhou et al.~\cite{zhou2018compressibility} highlighted the close connection between neural network compression and generalization. In~\cite{arora2018stronger}, the authors presented a compression method based on the Johnson-Lindenstrauss (JL) Lemma~\cite{johnson1984extensions} and proved sharper generalization bounds based on succinct reparameterizations, i.e., compression, of the original neural network. Within a similar context,~\cite{zhang2016understanding} and~\cite{neyshabur2017exploring} explored various training techniques that are commonly believed to help generalization, however, the presented empirical evidence suggests otherwise. Moreover, they point out that the number of parameters in modern neural network architectures clearly exceed the number of available training data points, thus suggesting parameters are highly redundant and thus there is a high potential in reducing the number of parameters. Generalization has also been investigated extensively in various other contexts~\cite{dziugaite2017computing,neyshabur2017pac,kawaguchi2017generalization,bartlett2017spectrally,arora2018stronger}. Building upon the works of of~\cite{arora2018stronger} and~\cite{zhou2018compressibility}, our work extends our theoretical compression results to establish instance-dependent and -independent generalization bounds that may provide novel insights on the generalization properties of neural networks.

\CB{TODO: Cite~\cite{frankle2018lottery}}
\CB{TODO: Rewrite}
Compared to~\cite{arora2018stronger}, which also introduces data-aware bounds that may yield sharper generalization bounds, our compression framework holds for any data point from the input distribution -- not just the training data -- thus our obtained generalization bounds are also valid for data outside the training data. Our method has the added benefit of generating sparse weight matrices that, in addition to alleviating space requirements, may also enable significant speed ups in inference via the use of sparse linear algebra algorithms~\cite{yuster2005fast}.


% LENGTHY VERSION OF COMPRESSION

\paragraph{Low-rank Decompositions}
Work in this category is mostly based on the observation that the trained weight matrices have a few dominant singular values, which implies that the weight matrices can be efficiently and accurately represented using their low-rank counterparts consisting only of the first few singular vectors.
Denil et al.~\cite{Denil2013} were among the first to empirically establish that there is significant redundancy in the parameters of deep neural networks. \IG{I wonder if this is true, as Denil's paper came way after the optimal brain damage paper.}
Denton et al.~\cite{Denton14} extend the notion of exploiting parameter redundancy to speed up test-time evaluation of Convolutional Neural Networks (CNNs). They compress the convolutional layers of a neural network by generating appropriate low-rank approximations of convolutional weight tensors to improve test-time performance. \cite{jaderberg2014speeding} and~\cite{kim2015compression} introduce a similar paradigm based on low-rank decompositions of convolutional tensors.

\cite{tai2015convolutional} propose a compression strategy based on low-rank tensor decompositions for accelerating CNNs and reducing their space requirement. In this work low-rank tensors are enforced through regularization during training. They also note that empirical evidence suggests that low-rank regularization can aid generalization.
%Unlike prior iterative algorithms for computing the decomposition, they prove that there exists a closed-form solution for a particular form of low-rank decomposition (as in \cite{jaderberg2014speeding}), thus, their algorithm efficiently finds the globally optimal solution by using SVD at its core.  
Similarly,~\cite{alvarez2017compression} and~\cite{ioannou2015training} also investigate regularization during training to enforce weight tensors that are suitable for low-rank approximations.
Recently, Yu et al.~\cite{yu2017compressing} introduce an SVD-free, greedy-bilateral scheme for deep compression that simultaneously generates a low-rank and sparse approximation of the weight matrices with feature map reconstruction. Despite their empirical effectiveness in compressing neural networks, these works provide no performance guarantees on the quality of their approximations.


\paragraph{Feature Hashing and Weight Sharing}
Weinberger et al.~\cite{Weinberger09} and Shi et al. ~\cite{shi2009hash} introduce the \emph{hashing-trick} where a hash function is used to hash a high dimensional input vector into a lower dimensional feature space -- much similar to the (optimal) dimensionality-reduction provided by the Johnson-Lindenstrauss 
lemma~\cite{johnson1984extensions,larsen2016optimality}. The authors provide empirical evidence of effectiveness and prove strong concentration bounds on the dot-product preserving nature of their compression, although
tighter theoretical bounds for the results in above work can be obtained via Sparse Johnson-Lindenstrauss Transforms~\cite{dasgupta2010sparse,kane2014sparser}. 
HashedNets~\cite{Chen15Hash} and FreshNets~\cite{Chen15Fresh} build upon the idea of feature hashing and introduce a weight-sharing scheme where a hash function is used to randomly group network connections so that all connections within one group share the same parameter value. %This enables neural network training with a much smaller set of parameters, while preserving the expressiveness of the network. 
A different approach to weight-sharing is explored in~\cite{ullrich2017soft}.
Although the papers do not investigate the theoretical properties of their approach, they present empirical evidence that networks can be compressed using random weight-sharing.

\paragraph{Structured Matrices} 
Building upon the idea of weight-sharing, these papers consider the case when the weight matrices contain a regular structure, thus reducing the effective number of parameters. Examples of such matrices include low  displacement rank matrices, which are investigated in~\cite{Zhao17} and independently in~\cite{sindhwani2015structured}, as well as circular matrices~\cite{cheng2015exploration}. Both approaches show empirical evidence that neural networks containing such structured matrices can still be trained effectively. In~\cite{choromanska2016binary} structured binary embeddings of weight matrices are considered, whereas~\cite{wen2016learning} considers a regularization approach to enforce structured weight matrices during training. 
